Wasm-bpf: Streamlining eBPF Deployment in Cloud Environments with WebAssembly

The extended Berkeley Packet Filter (eBPF) is extensively utilized for observability and performance analysis in cloud-native environments. However, deploying eBPF programs across a heterogeneous cloud environment presents challenges, including compatibility issues across different kernel versions, operating systems, runtimes, and architectures. Traditional deployment methods, such as standalone containers or tightly integrated core applications, are cumbersome and inefficient, particularly when dynamic plugin management is required. To address these challenges, we introduce Wasm-bpf, a lightweight runtime on WebAssembly and the WebAssembly System Interface (WASI). Leveraging Wasm platform independence and WASI standardized system interface, with enhanced relocation for different architectures, Wasm-bpf ensures cross-platform compatibility for eBPF programs. It simplifies deployment by integrating with container toolchains, allowing eBPF programs to be packaged as Wasm modules that can be easily managed within cloud environments. Additionally, Wasm-bpf supports dynamic plugin management in WebAssembly. Our implementation and evaluation demonstrate that Wasm-bpf introduces minimal overhead compared to native eBPF implementations while simplifying the deployment process.

==> case_study.tex <==
\subsection{Case Study}

\subsection{eBPF makes WASI more secure}
More possible system call filtering mechanism inside WASI by extending the BPF syscall in WASI. 

LSM policy

\subsection{eBPF help debug the WASM Runtime}
case study
